A Long Look at the Be/X-Ray Binaries of the Small Magellanic Cloud

We have monitored 41 Be/X-ray binary systems in the Small Magellanic Cloud over ~9 years using PCA-RXTE data from a weekly survey program. The resulting light curves were analysed in search of orbital modulations with the result that 10 known orbital ephemerides were confirmed and refined, while 10 new ones where determined. A large number of X-ray orbital profiles are presented for the first time, showing similar characteristics over a wide range of orbital periods. Lastly, three pulsars: SXP46.4, SXP89.0 and SXP165 were found to be misidentifications of SXP46.6, SXP91.1 and SXP169, respectively.

==> tab1.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
%\makeatother
%\ptlandscape
\begin{deluxetable}{lcc}
\tabletypesize{\scriptsize}
%\rotate
\tablecolumns{3}
\tablewidth{0pt}
\tablecaption{\rxte 's \smc\ survey pointing positions \label{table_pointings}}
\tablehead{ \colhead{Name} & \colhead{RA (\degree)} & \colhead{Dec (\degree)} }
\startdata
  1a             &   00 52 07.8   &   \minus72 25 43.3  \\
  1b             &   00 51 04.0   &   \minus72 13 44.0  \\
  1c (SMC X-3)   &   00 54 54.8   &   \minus72 26 40.9  \\
  1/A            &   00 53 53.0   &   \minus72 26 42.0  \\
  2              &   01 05 00.0   &   \minus72 06 00.0  \\
  3              &   01 15 00.0   &   \minus73 06 00.0  \\
  4              &   00 50 44.6   &   \minus73 16 04.8  \\
  5              &   00 50 00.0   &   \minus73 06 00.0  \\
  B              &   01 05 00.0   &   \minus72 06 21.6  \\
  C              &   01 15 00.0   &   \minus73 24 59.8  \\
  D              &   00 50 00.0   &   \minus73 06 00.0  \\
  X              &   01 05 00.0   &   \minus72 06 00.0  \\
  SMC X-2        &   00 54 33.3   &   \minus73 41 04.2  \\
\enddata
\end{deluxetable}


==> tab2.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
%\makeatother
%\ptlandscape
\begin{deluxetable}{lcc}
\tabletypesize{\scriptsize}
%\rotate
\tablecolumns{3}
\tablewidth{0pt}
\tablecaption{Parameters used for the Lomb-Scargle periodogram \label{table_LS_params}}
\tablehead{ \colhead{} & \colhead{Group 1} & \colhead{Group 2} }
\startdata
  $P_{\rm min}$ (s)  &  0.5             &  10 \\
  $P_{\rm max}$ (s)  &  1000            &  3000 \\
  $\Delta f$ (Hz)    &  10\supersm{-5}  &  $5 \times 10^{-7}$ \\
  Search range (s)   &  0.5\sd40        &  40\sd3000 \\
\enddata
\end{deluxetable}

